AraT5: Text-to-Text Transformers for Arabic Language Generation

Transfer learning with a unified Transformer framework (T5) that converts all language problems into a text-to-text format was recently proposed as a simple and effective transfer learning approach. Although a multilingual version of the T5 model (mT5) was also introduced, it is not clear how well it can fare on non-English tasks involving diverse data. To investigate this question, we apply mT5 on a language with a wide variety of dialects--Arabic. For evaluation, we introduce a novel benchmark for ARabic language GENeration (ARGEN), covering seven important tasks. For model comparison, we pre-train three powerful Arabic T5-style models and evaluate them on ARGEN. Although pre-trained with ~49 less data, our new models perform significantly better than mT5 on all ARGEN tasks (in 52 out of 59 test sets) and set several new SOTAs. Our models also establish new SOTA on the recently-proposed, large Arabic language understanding evaluation benchmark ARLUE (Abdul-Mageed et al., 2021). Our new models are publicly available. We also link to ARGEN datasets through our repository: https://github.com/UBC-NLP/araT5.

==> RW_Full.tex <==

 \section{Related Work}\label{sec:RW}


In this section, we will provide a brief description of  the MLM  which covered Arabic language.
 \subsection{Multilingual LMs}\label{sec:Mult_LM}
\noindent\textbf{mBERT} mBERT is the multilingual version of BERT~\cite{devlin2019bert} which is
 a multi-layer bidirectional encoder representations from Transformers trained with a masked language modeling.~\cite{devlin2019bert} present two architecture BERT$_{Base}$ with $12$ layers (transformer blocks), $12$ attention heads, and $110$ million parameters. the second architecture was BERT$_{Large}$ comes  with $24$ layers, $16$ attention heads, and $340$ million parameters.  BERT models were trained on  English Wikipedia~\footnote{\href{https://www.wikipedia.org/}{https://www.wikipedia.org/}} and  BooksCorpus~\cite{Zhu_2015_ICCV}. mBERT  it is trained on Wikipedia for $104$ languages (including Arabic $\sim153$M tokens ) with  $12$ layers, $12$ attention heads, $768$ hidden units each and $110$M parameters.  \\
 
\noindent\textbf{XLM-R} ~\cite{conneau2019unsupervised} is a transformer-based multilingual masked language model pre-trained on  more than $2$ TB  of filtered CommonCrawl data in $100$ languages, including Arabic ($2.9$B tokens).  XLM-R use a Transformer model \cite{vaswani2017attention} trained with a multilingual masked language models XLM \cite{lample2019cross}.  It comes in two sizes and architectures:  XLM-R\textsubscript{Base} \textit{Base} and   XLM-R\textsubscript{Large}. XLM-R\textsubscript{Base}  architecture which contains $12$ layers, $12$ attention heads, $768$ hidden units  and  $270$M parameters. The  XLM-R\textsubscript{Large}  architecture has   $124$ layers, $16$ attention heads, $1024$ hidden units  and  $550$M parameters.   While both XLM-R models use the same masking objective as BERT, they do not include the next sentence prediction objective used in BERT.   Recently, XLM-R obtains state-of-the-art performance on  sequence labeling, cross-lingual classification, and question answering. \\
 

 
\noindent\textbf{mT5}~\cite{xue2020mt5} is the multilingual version of \textbf{T}ext-\textbf{t}o-\textbf{T}ext \textbf{T}ransfer \textbf{T}ransformer model (T5)   \cite{raffel2019exploring}.  The T5 model architecture is essentially an encoder-decoder Transformer~\cite{vaswani2017attention} similar in configuration and size to a BERT$_{Base}$~\cite{devlin2019bert}, with some architectural modifications including applying a normalization layer  before a sub block and  adding an initial input to the sub-block output. The basic idea behind  this  model is to  treat every  text-based language task as a “text-to-text” problem, (i.e. taking text format as input and producing new text format as output), where   a multi-task learning  is applied to several  NLP tasks: question answering, document summarization, machine translation, and sentiment classification.  mT5  is trained on the ``Multilingual Colossal Clean Crawled Corpus" (or mC4 for short), which is  $\sim26.76$TiB for $101$ languages generated from $71$ Common Crawl dumps. \\


\noindent\textbf{mBART}~\cite{liu2020multilingual} is  a  multilingual sequence-to-sequence denoising auto-encoder pre-trained for neural machine translation task. mBART is trained on large-scale monolingual corpora in many languages using the BART objective~\cite{lewis2019bart}.

 \subsection{Arabic LMs}\label{sec:Arabic_LM}

 


\noindent\textbf{AraBERT}~\cite{antoun2020arabert} is an Arabic pre-trained language model based on the  BERT$_{Base}$ architecture~\cite{devlin2019bert}  configuration. AraBERT ~\cite{antoun2020arabert}  was trained on $23$GB of Arabic text, comprising more than $70$M sentences and 3B words. In fact,   AraBERT is trained on  Arabic Wikipedia, the Open Source International dataset (OSIAN) \cite{zeroual2019osian} ($3.5$M news articles from  $24$ Arab countries), and $1.5$B words Corpus  from \cite{elkhair-2016} ($5$M articles extracted from ten news sources). \newcite{antoun2020arabert} evaluate AraBERT on three Arabic downstream tasks. These are (1) sentiment analysis from 6 different datasets: HARD~\cite{elnagar2018hotel}, ASTD~\cite{nabil2015astd}, ArsenTD-Lev~\cite{baly2019arsentd}, LABR~\cite{aly2013labr}, and ArSaS~\cite{elmadany2018arsas}. (2) NER, with the ANERcorp~\cite{anercorp}, and  (3) Arabic QA, on Arabic-SQuAD~\cite{mozannar2019neural} and ARCD~\cite{mozannar2019neural} datasets. \\



\noindent\textbf{ARBERT}~\cite{abdul2020arbert} is a large scale pre-training masked language model focused on Modern Standard Arabic (MSA).ARBERT is trained on a collection of Arabic datasets comprising $61$GB of text  (6.2B tokens).  The same architecture as BERT\textsubscript{Base} was used: $12$ attention layers, each has $12$ attention heads and $768$ hidden dimensions, a vocabulary of $100$K WordPieces, making $\sim163$M parameters.  \\



\noindent\textbf{MARBERT}\cite{abdul2020arbert} iis a large scale pre-training masked language model focused on both Dialectal Arabic (DA) and MSA. This model is trained on a sample of 1B Arabic tweets ($128$GB of text, ~$15.6$B tokens). In this dataset  only  tweets with at least $3$ Arabic words are included, based on character string matching, regardless whether the tweet has non-Arabic string or not. MARBERT~ use the same a vocabulary size ($100$K WordPieces) and network architecture as ARBERT (BERT-base), but without the next sentence prediction (NSP) objective since tweets are short.



==> datasets/SA_datasets.tex <==

\begin{itemize}

\item \textbf{AJGT.} The Arabic Jordanian General Tweets (AJGT) dataset~\cite{alomari2017arabic} involves MSA and Jordanian tweets, with a balanced split of $900$ \textit{positive} posts and $900$ \textit{negative} posts (total=$1,800$).

\item \textbf{AraNET\textsubscript{Sent}}.
~\newcite{mageed-2020-aranet} collect $15$ datasets in both MSA and dialects from~\newcite{mageed2012awatif} (AWATIF), ~\newcite{mageed2014samar} (SAMAR),~\newcite{abdulla2013arabic,nabil2015astd,kiritchenko2016semeval,aly2013labr,salameh2015sentiment,rosenthal2017semeval,alomari2017arabic,mohammad2018semeval}, and~\newcite{baly2019arsentd}. These datasets involve varying numbers of sentiment categories: \textbf{binary} (\textit{negative} and \textit{positive}), \textbf{3-way} (\textit{negative}, \textit{neutral}, and \textit{positive}). Some of the datasets also have a \textit{subjective} language label.~\newcite{mageed-2020-aranet} combine the datasets for binary sentiment classification by reducing the different tags into the binary case (i.e., \textit{negative} and \textit{positive}) and removing data from all other labels, acquiring $126,766$ samples, which they split into 80\% ($100,599$), 10\% ($14,344$) and 10\% ($11,823$) for training, development, and test respectively. 

\item \textbf{AraSenTi-Tweet}. This is a collection of MSA and Saudi Arabic
tweets by~\newcite{al2017arasenti}. The $17,573$ dataset is manually annotated. The distribution of labels is as follows: $4,957$ \textit{positive},  $6,155$ \textit{negative}, $4,639$ \textit{neutral}, and $1,822$ \textit{mixed} sentences.

\item \textbf{ArSarcasm\textsubscript{Sent}}~\newcite{farha2020arabic} introduce ArSarcasm, a sarcasm dataset labeled with sentiment tags. ArSarcasm has $10,547$ tweets, of which $2,472$ taken from ASTD \cite{nabil2015astd} and $8,075$ from SemEval-2017 Task 4~\cite{rosenthal2017semeval}. ~\newcite{farha2020arabic} evaluate on the $3$ sentiment labels \textit{negative}, \textit{neutral}, and \textit{positive}.
 
\item \textbf{ArSAS}. The Arabic Speech Act and Sentiment (ArSAS) corpus~\cite{elmadany2018arsas} consists of $21,064$ tweets annotated with four labels:  \textit{positive}, \textit{negative}, \textit{neutral}, and \textit{mixed}. 


\item \textbf{ArSenD-Lev}. The Arabic Sentiment Twitter Dataset for LEVantine dialect (ArSenD-Lev)~\cite{baly2019arsentd} has $4,000$ tweets retrieved from the Levant region (i.e., Jordan, Lebanon, Palestine, and Syria). Sentiment is labeled on a 5-point scale, with $835$ \textit{positive}, $397$ \textit{very positive}, $885$ \textit{neutral}, $1,253$ \textit{negative,} and $630$ \textit{very negative}.

\item \textbf{ASTD.} This is a collection of $10,006$  Egyptian tweets annotated with the labels positive (n=$799$), \textit{negative} (n=$1,684$),  \textit{objective} (n=$832$), and \textit{neutral} (n=$6,691$) by ~\newcite{nabil2015astd}.

\item \textbf{AWATIF}. A multi\-genre MSA dataset~\cite{mageed2012awatif} consisting of $2,855$ sentences of newswire stories from Part 1, V3 of the Penn Arabic TreeBank,\footnote{\href{https://catalog.ldc.upenn.edu/LDC2005T20}{https://catalog.ldc.upenn.edu/LDC2005T20}.} $5,342$ sentences from $30$ Wikipedia talk pages, and $2,532$ threaded conversations from $7$ web forums.


\item \textbf{BBNS \&  SYTS}.  The {\bf BBN} blog posts {\bf S}entiment (BBNS) and {\bf S}yria {\bf T}weets {\bf S}entiment  (SYTS)  are introduced by \newcite{salameh2015sentiment}. BBNS comprises $1,200$ Levantine dialectal sentences extracted from the BBN Arabic-Dialect/English Parallel Text.\footnote{\href{ https://catalog.ldc.upenn.edu/LDC2012T09}{ https://catalog.ldc.upenn.edu/LDC2012T09}.}  SYTS consist of $2,000$ Levantine Arabic tweets. Both BBNS and  SYTS are manually annotated with tags from the set \textit{\{negative, positive, neutral\}}.  

\item \textbf{CAMel\textsubscript{Sent}}.~\newcite{obeid2020camel} merge training and development data from ArSAS~\cite{elmadany2018arsas}, ASTD~\cite{nabil2015astd}, SemEval~\cite{rosenthal2017semeval}, and ArSenTD~\cite{al2017arasenti} to create a new training dataset ($\sim	24$K). For evaluation, they report performance on the independent test set from each of these sources.


\item \textbf{HARD}. The Hotel Arabic Reviews Dataset (HARD)~\cite{elnagar2018hotel} consists of $93,700$ hotel reviews, each with a rating of $1$-$5$ stars. The reviews are  written in MSA and DA. Reviews with $1$ and $2$ stars are treated as \textit{negative} and those with $4$ and $5$ stars as \textit{positive}. Reviews with $3$ stars reviews are removed from the dataset. Overall, there are $46.8$K for each of the \textit{positive} and \textit{negative} classes. 
% \note[mam]{Is the $93,700$ total before or after removing neutral?}

\item \textbf{LABR}. The Large Arabic Book Review Corpus~\cite{aly2013labr} has $63,257$ book reviews from Goodreads, the book readers social network.\footnote{\href{www.goodreads.com}{www.goodreads.com}.} The reviews are rated with a $1$-$5$ stars scale. Posts with $1$-$2$ stars are treated as \textit{negative}, those with $3$ starts as \textit{neutral}, and those with $3$-$5$ as \textit{positive}.

\item \textbf{Twitter$_{\bf Abdullah}$.}\footnote{For ease of reference, we assign a name to this and other unnamed datasets.} This is a dataset of $2,000$ MSA and Jordanian Arabic tweets manually labeled by \newcite{abdulla2013arabic}. The dataset is balanced, with $1,000$ \textit{positive} and $1,000$ \textit{negative} tweets.
%\note[mam]{We should prepare a table with the sentiment data splits where we put the distribution of classes. I think we did this in AraNet paper, but we have more datasets here. \abdu{created table of data distribution check Table\ref{tab:SA_distrib}}}



\item \textbf{Twitter$_{\bf Saad}$.} This dataset is released by Moatez Saad in 2019 and is available on Kaggle.\footnote{\href{https://www.kaggle.com/mksaad/arabic-sentiment-twitter-corpus}{www.kaggle.com/mksaad/arabic-sentiment-twitter-corpus}.} The dataset is collected using an emoji lexicon as a proxy for sentiment. In total, it  has  $29.8$K \textit{positive} and $28.7$K \textit{negative} tweets.
% \note[mam]{$58$K total: how many pos and how many neg?}% ($47$K training and $11$K test) annotated in positive and negative labels.

\note[mam]{Please add this info.}%In addition to sentiment labels on a 5-point scale, the following information is provided for each tweet: topic, country of origin, and whether the expressed sentiment is implicit or explicit.

\note[mam]{Where is SAMAR dataset here?}

\item \textbf{SemEval-2017}. The SemEval-2017 sentiment analysis in Arabic Twitter task~\cite{rosenthal2017semeval} provides data for $3$ sentiment analysis sub-tasks. These included on $2$ classes (\textit{negative} and \textit{positive}) with $9,500$ tweets, $3$ classes (\textit{negative}, \textit{positive}, and \textit{neutral}) with $3,400$ tweets, and $5$ classes (\textit{strongly negative}, \textit{negative}, \textit{neutral}, \textit{positive} and \textit{strongly positive}) with $9,450$ tweets.


%\note[mam]{Where is SYST dataset here? OK I see it is listed with BBN.}



\end{itemize}


==> tables/AraLG_QG.tex <==

\begin{table}[ht]
 \centering
 \footnotesize

 \begin{tabular}{lrcc}
 \toprule
\textbf{Split} & \#\textbf{Art./Tit.}   &  \textbf{Avg Art.} & \textbf{Avg Tit. }\\
\toprule
\textbf{TRAIN}     &    $93.3$K & $256.46$   &$10.06$  \\
\textbf{DEV}        &   $11.7$K  & $253.11$    & $10.03$  \\
\textbf{TEST}        &  $11.7$K & $260.32$   & $10.03$   \\
\cline{1-4}
\textbf{Total}        &  $116.6$K & $256.63$   &$10.04$   \\
\toprule 
\end{tabular}
\caption{\footnotesize Main characteristics of  AraGen\textsubscript{TG} data splits. For each split, we provide the number of article-title pairs and the average length of the articles and titles.  \hl{DONE} }  \label{tab:arnews_tg}

    \end{table}

==> tables/DEV_DA_multi_tasks.tex <==
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule 
\textbf{Dataset}     & \textbf{Setting} & \textbf{mT5} & \textbf{AraT5\textsubscript{Tweet}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{AraT5\textsubscript{}} \\
% \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{Acc/EM}                       & \textbf{FPN/F1}                      & \textbf{Acc/EM}             & \textbf{FPN/F1}            & \textbf{Acc/EM}                 & \textbf{FPN/F1}                 & \textbf{Acc/EM}                & \textbf{FPN/F1}               & \textbf{Acc/EM}                   & \textbf{FPN/F1}                 \\
\toprule 
\multicolumn{1}{c}{\multirow{2}{*}{ARLUE\textsubscript{Dia-B}}}
   & S                               & $88.47$ / $88.04$                      & $89.73$ / $89.37$                           &$\bf90.31$ / $\bf89.97$                & $90.07$ / $89.74$                                     \\ 
   &M                                & $89.02$ / $88.30$	& $90.02$ / $89.71$                          & $89.96$ / $89.64$	& $89.98$ / $89.64$                                    \\\hline
\multicolumn{1}{c}{\multirow{2}{*}{ARLUE\textsubscript{Dia-R}}}                                         & S                               & $88.30$ / $87.93$                      & $90.12$ / $89.65$                           & $91.17$ / $90.80$                         & $91.13$ / $90.87$                                           \\
&M                                & 89.12 / 88.10 &	91.53 / 91.17                           & $91.42$ / $91.15$ &	$\bf91.51$ / $\bf91.24$                                    \\\hline
\multicolumn{1}{c}{\multirow{2}{*}{ARLUE\textsubscript{Dia-C}}}                                       & S                               & $44.92$ / $35.39$                      & $51.80$ / $39.04$                           & $51.30$ / $40.19$                         & $51.53$ / $40.21$                             \\
   &M                                & $44.98$ / $35.50$	& $51.92$ / $40.17$                          & $51.62$ / $40.25$	& $\bf52.02$ / $\bf40.55$                  \\
    \toprule             
\end{tabular}%
}
\caption{Performance of our models on ARLUE Dialects DEV datasets on single and multi tasks setting (Acc / F$_1$). We copied single tasks results from Table~\ref{tab:ArBench_res_dev} in this table for comparison. \textbf{S}: Single Task.\textbf{ M}:Multi-task.}  \label{tab:ArBench_multi_da_dev}
\end{table}



==> tables/DEV_SM_multi_tasks.tex <==
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule 
\textbf{Dataset}     & \textbf{S/M} & \textbf{mT5} & \textbf{AraT5\textsubscript{Tweet}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{AraT5\textsubscript{}} \\
% \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{Acc/EM}                       & \textbf{FPN/F1}                      & \textbf{Acc/EM}             & \textbf{FPN/F1}            & \textbf{Acc/EM}                 & \textbf{FPN/F1}                 & \textbf{Acc/EM}                & \textbf{FPN/F1}               & \textbf{Acc/EM}                   & \textbf{FPN/F1}                 \\
\toprule 
\multicolumn{1}{c}{\multirow{2}{*}{Age}}
   & S                                & $60.86$ / $61.05$	&	$62.29$ / $62.48$	&	$63.26$ / $63.41$	&	$63.50$ / $63.66$                                   \\ 
   &M                                & $61.44$ /$61.52$	&	$64.22$ /$64.39$	&	$63.96$ /$64.13$	&	$\bf63.97$ /$\bf64.05$                                   \\\hline
   
   \multicolumn{1}{c}{\multirow{2}{*}{Dangerous}}
   & S                                & $80.00$ / $69.57$	&	$82.28$ / $74.99$	&	$80.98$ / $70.89$	&	$79.51$ / $72.10$                                 \\ 
   &M                                & $79.02$ / $71.50$	&	$82.11$ / $76.07$	&	$\bf82.93$ / $\bf75.41$	&	$81.30$ / $74.82$                                    \\\hline

\multicolumn{1}{c}{\multirow{2}{*}{Emotion}}
   & S                                & $71.32$ / $70.25$	&	$73.30$ / $71.93$	&	$73.85$ / $73.37$	&	$\bf74.18$ / $\bf73.56$                                   \\ 
   &M                                & $69.89$ / $68.49$	&	$72.53$ / $71.34$	&	$72.64$ / $71.77$	&	$72.97$ / $72.13$                                    \\\hline
\multicolumn{1}{c}{\multirow{2}{*}{Gender}}
   & S                                & $72.05$ / $71.83$	&	$72.27$ / $72.06$	&	$73.83$ / $73.56$	&	$73.38$ / $73.24$                                     \\ 
   &M                                & $72.66$ / $72.35$	&	$74.34$ / $74.15$	&	$\bf74.45$ / $\bf74.32$	&	$74.44$ / $74.31$                                    \\\hline
\multicolumn{1}{c}{\multirow{2}{*}{Hate}}
   & S                                & $95.70$ / $76.71$	&	$96.60$ / $80.22$	&	$\bf96.80$ / $\bf82.83$	&	$96.50$ / $81.40$                                    \\ 
   &M                                & $95.70$ / $76.71$	&	$96.40$ / $80.69$	&	$96.00$ / $78.12$	&	$96.60$ / $80.22$                                    \\\hline    
\multicolumn{1}{c}{\multirow{2}{*}{Irony}}
   & S                                & $82.88$ / $82.83$	&	$84.37$ / $84.33$	&	$\bf84.86$ / $\bf84.85$	&	$83.87$ / $83.81$                                     \\ 
   &M                                & $81.89$ /$81.88$	&	$84.12$ /$84.12$	&	$84.62$ /$84.54$	&	$\bf85.61$ /$\bf85.58$                                    \\\hline
\multicolumn{1}{c}{\multirow{2}{*}{Offensive}}
   & S                                & $93.70$ / $88.92$	&	$95.20$ / $91.76$	&	$95.20$ / $91.90$	& $\bf95.60$ /$\bf92.48$                                     \\ 
   &M                                & $92.20$ / $86.85$	&	$94.60$ / $91.01$	&	$94.70$ / $90.92$	&		$93.70$ / $89.53$                                    \\\toprule

% \multicolumn{1}{c}{\multirow{2}{*}{Sarcasm}}
%   & S                                & --	&	--	&	--	&	--                                     \\ 
%   &M                                & --                      &--                           & --	& --                                    \\\toprule 
\textbf{ARLUE\textsubscript{SM}\textsuperscript{$\dagger$}     }                                       
&    S	                         & $79.50$ / $74.45$	& $80.90$ / $76.82$	& $81.25$ / $\bf77.26$	& $80.93$ / $77.18$                              \\
&M                                & $78.97$ / $74.19$	& $81.19$ / $77.40$	& $81.33$ / $77.03$	& $81.23$ / $\bf77.23$ \\
\toprule             
\end{tabular}%

}
\caption{Performance of our models on ARLUE Social Meaning (SM) DEV datasets on single and multi tasks setting (Acc / F$_1$). \textbf{S}: Single Task.\textbf{ M}:Multi-task.}  \label{tab:ArBench_multi_sm_dev}
\end{table}

==> tables/DEV_tab_ArBench_res.tex <==
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule 
\textbf{Dataset}     & \textbf{SOTA} & \textbf{mT5} & \textbf{AraT5\textsubscript{Tweet}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{AraT5\textsubscript{}} \\
% \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{Acc/EM}                       & \textbf{FPN/F1}                      & \textbf{Acc/EM}             & \textbf{FPN/F1}            & \textbf{Acc/EM}                 & \textbf{FPN/F1}                 & \textbf{Acc/EM}                & \textbf{FPN/F1}               & \textbf{Acc/EM}                   & \textbf{FPN/F1}                 \\
\toprule 
ARLUE\textsubscript{Senti}$^\star$                                           & $92.82$ / $93.50$                                & $92.46$ / $93.50$                      & $92.79$ / $93.50$                           & $\bf93.44$ / $\bf94.00$                & $93.30$ / $94.00$                                   \\
ARLUE\textsubscript{SM}\textsuperscript{$\dagger$}                                            & $80.49$ / $75.72$                                &

$79.50$ / $74.45$	& $80.90$ / $76.82$	& $\bf81.25$ / $\bf77.26$	& $80.93$ / $77.18$ \\
% 69.56 / 65.15                      & 70.79 / 67.22                           & 71.10 / 67.60                         & 70.82 / 67.53                                   \\
ARLUE\textsubscript{Topic}                                           & $91.52$ / $92.50$                                & $91.77$ / $93.11$                      & $91.60$ / $92.89$                           & $\bf92.84$ / $\bf94.02$                & $92.62$ / $94.01$                                      \\
ARLUE\textsubscript{Dia-B}                                         & $90.05$ / $89.72$                                & $88.47$ / $88.04$                      & $89.73$ / $89.37$                           & $\bf90.31$ / $\bf89.97$                & $90.07$ / $89.74$                                     \\
ARLUE\textsubscript{Dia-R}                                         & $90.04$ / $89.67$                                & $88.30$ / $87.93$                      & $90.12$ / $89.65$                           & $\bf91.17$ / $90.80$                         & $91.13$ / $\bf90.87$                                           \\
ARLUE\textsubscript{Dia-C}                                        & $45.37$  / $35.94$                                & $44.92$ / $35.39$                      & $\bf51.80$ / $39.04$                           & $51.30$ / $40.19$                         & $51.53$ / $\bf40.21$                             \\
% ARLUE\textsubscript{NER}                                            & 97.97 / 85.56                                & - / -                          &- / -                               &- / -                             & - / -   \\                  

ARLUE\textsubscript{QA}$^\ddagger$                                             & $37.14$ / $\bf57.93$               & $33.46$	/ $51.83$                          & $27.47$ / $46.54$                               & $\bf37.33$ / $57.50$                             & $35.59$ / $56.25$\\    
\hline
Average     &  $75.35$ / $76.43$	& $74.13$ / $74.89$	& $74.92$ / $75.40$	& $\bf76.81$ / $\bf77.68$	& $76.45$ / $77.47$                    \\\toprule 
\textbf{ARLUE\textsubscript{Score}}     
            & $75.89$	& 	$74.51$	& 	$75.16$	& $\bf77.24$	& $76.96$	 \\     \toprule             
\end{tabular}%
}
\caption{Performance of our models on ARLUE DEV datasets (Acc / F$_1$). $^\star$ Metric for ARLUE\textsubscript{Senti} is Acc/ F\textsubscript{1}\textsuperscript{PN}. $^*$Metric for ARLUE\textsubscript{QA} is Exact Match (EM) /  F$_1$.$^\dagger$ Metric for ARLUE\textsubscript{Senti} is F\textsubscript{1}\textsuperscript{PN}. \textbf{SOTA:} MARBERT \cite{abdul2020arbert}}  \label{tab:ArBench_res_dev}
\end{table}


% ####################################################
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccccccccc}
% \toprule
% % \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{XLM-R\textsubscript{B}}} & \multicolumn{2}{c}{\textbf{XLM-R\textsubscript{L}}} & \multicolumn{2}{c}{\textbf{AraBERT}} & \multicolumn{2}{c}{\textbf{ARBERT}} & \multicolumn{2}{c}{\textbf{MARBERT}} & \multicolumn{2}{c}{\textbf{MARBERT(v2)}} \\ \cline{2-17} 
% %                          & \textbf{Acc/EM$^*$}          & $\bf F_1$          & \textbf{Acc/EM$^*$}           & $\bf F_1$          & \textbf{Acc/EM$^*$}           & $\bf F_1$           & \textbf{Acc/EM$^*$}           & $\bf F_1$           & \textbf{Acc/EM$^*$}            & $\bf F_1$           & \textbf{Acc/EM$^*$}           & $\bf F_1$           & \textbf{Acc/EM$^*$}            & $\bf F_1$           & \textbf{EM$^*$}              & $\bf F_1$            \\ 
                         
% %     \toprule                     
% \textbf{Dataset}&\textbf{mBERT} & \textbf{XLM-R\textsubscript{B}} & \textbf{XLM-R\textsubscript{L}} & \textbf{AraBERT} & \textbf{ARBERT} & \textbf{MARBERT} & \textbf{MARBERT (v2)} \\
% % \cline{2-15}
% %                          &\textbf{Acc/EM$^*$}      & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}      &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}      &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}      &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}       &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}      &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}       &\textbf{Acc/EM$^*$}         & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}         \\
% \toprule
% ArBench\textsubscript{Senti}$^\star$           & $79.02$ / $79.50$       & $92.17$ / $93.00$       & $93.18$ / $\bf 94.00$       & $78.26$ / $78.50$        & $87.96$ / $88.50$       & $\bf 93.30$  / $\bf 94.00$        & $\bf 93.30$ / $\bf 94.00$          \\
% ArBench\textsubscript{SM}\textsuperscript{$\dagger$}              & $77.76$ / $69.88$       & $79.81$ / $71.19$       & $80.01$ / $73.00$       & $78.84$ / $72.03$        & $80.39$ / $74.22$       & $\bf82.35$ / $\bf77.13$       & $76.34$ / $\bf77.13$           \\
% ArBench\textsubscript{Topic}           & $90.88$ / $92.12$       & $90.90$ / $91.81$       & $\bf 92.24$ / $\bf 93.40$       & $92.15$ / $92.97$        & $90.81$ / $92.65$       & $89.67$ / $90.97$        & $90.07$ / $91.54$          \\
% ArBench\textsubscript{Dia-B}          & $85.52$ / $84.88$       & $86.54$ / $85.98$       & $87.82$ / $87.17$       & $87.74$ / $87.21$        & $88.31$ / $87.74$       & $88.72$ / $88.19$        & $\bf 88.47$ /  $\bf 87.87$          \\
% ArBench\textsubscript{Dia-R}          & $86.45$ / $85.89$       & $86.00$ / $85.46$       & $86.97$ / $86.54$       & $87.30$ / $86.92$        & $88.85$ / $88.49$       & $\bf 90.94$ / $\bf 90.65$        &$90.04$ / $89.67$            \\
% ArBench\textsubscript{Dia-C}         & $42.80$ / $35.23$       & $42.67$ / $35.40$       & $41.94$ / $34.98$       & $\bf 39.71$ / $33.56$        & $44.44$ / $36.87$       & $45.89$ / $37.69$        & $\bf 47.49$ / $38.53$          \\
% ArBench\textsubscript{NER}             & $95.90$ / $69.06$       & $96.02$ / $73.27$       & $96.13$ / $\bf 74.94$       & $96.76$ / $76.19$        & $97.00$ / $76.83$       & $96.38$ / $71.93$        & $\bf 96.75$ / $74.70$          \\
% ArBench\textsubscript{QA}$^\ddagger$              & $34.34$ / $55.74$       & $34.62$ / $56.67$       & $39.37$ / $\bf 63.12$       & $36.31$ / $58.10$        & $36.29$ / $57.81$       & $29.13$ / $48.83$        & $\bf 40.47$ / $62.09$          \\
% % \cdashline{2-8}	
% \hline
% Average  & $74.08$ / $71.54$       & $76.09$ / $74.10$       &$77.21$ / $75.89$       & $74.63$ / $73.19$        & $76.76$ / $75.39$       & $77.05$ / $74.92$        & $\bf77.87$  / $\bf 76.94$    \\
% 	\toprule		
% \textbf{ArBench\textsubscript{Score}}  & $72.81$       & $75.09$       &$76.55$       & $73.91$        & $76.07$       & $75.99$        & $\bf77.40$    \\
% \toprule
% \end{tabular}%
% }
% \caption{\small{Performance of our models on ArBench on (Acc / F$_1$). $^\star$ Metric for ArBench\textsubscript{Senti} is Acc/ F\textsubscript{1}\textsuperscript{PN}. $^\dagger$ ArBench\textsubscript{SM} results is the average score across the social meaning tasks described in Table~\ref{tab:SM_res}.} $^\ddagger$~Metric for ArBench\textsubscript{QA} is Exact Match (EM) / F$_1$. }
% \label{tab:Arbench_res}
% \end{table*}


% % % Please add the following required packages to your document preamble:
% % % \usepackage{multirow}
% % % \usepackage{graphicx}
% % \begin{table*}[]
% % \centering
% % \renewcommand{\arraystretch}{1.2}
% % \resizebox{\textwidth}{!}{%
% % \begin{tabular}{lcccccccccccccc}
% % \toprule
% % % \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{XLM-R\textsubscript{B}}} & \multicolumn{2}{c}{\textbf{XLM-R\textsubscript{L}}} & \multicolumn{2}{c}{\textbf{AraBERT}} & \multicolumn{2}{c}{\textbf{ARBERT}} & \multicolumn{2}{c}{\textbf{MARBERT}} & \multicolumn{2}{c}{\textbf{MARBERT(v2)}} \\ \cline{2-17} 
% % %                          & \textbf{Acc/EM$^*$}          & $\bf F_1$          & \textbf{Acc/EM$^*$}           & $\bf F_1$          & \textbf{Acc/EM$^*$}           & $\bf F_1$           & \textbf{Acc/EM$^*$}           & $\bf F_1$           & \textbf{Acc/EM$^*$}            & $\bf F_1$           & \textbf{Acc/EM$^*$}           & $\bf F_1$           & \textbf{Acc/EM$^*$}            & $\bf F_1$           & \textbf{EM$^*$}              & $\bf F_1$            \\ 
                         
% % %     \toprule                     
% % \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{XLM-R\textsubscript{B}}} & \multicolumn{2}{c}{\textbf{XLM-R\textsubscript{L}}} & \multicolumn{2}{c}{\textbf{AraBERT}} & \multicolumn{2}{c}{\textbf{ARBERT}} & \multicolumn{2}{c}{\textbf{MARBERT}} & \multicolumn{2}{c}{\textbf{MARBERT (v2)}} \\ \cline{2-15}
% %                          &\textbf{Acc/EM$^*$}      & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}      &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}      &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}      &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}       &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}      &\textbf{Acc/EM$^*$}       & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}       &\textbf{Acc/EM$^*$}         & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}}         \\
% % \toprule
% % ArBench\textsubscript{Senti}           & $79.02$       & $79.50$       & $92.17$        & $93.00$       & $93.18$        & $\bf 94.00$       & $78.26$        & $78.50$        & $87.96$        & $88.50$       & $\bf 93.30$        & $\bf 94.00$        & $\bf 93.30$          & $\bf 94.00$          \\
% % ArBench\textsubscript{Topic}           & $90.88$       & $92.12$       & $90.90$        & $91.81$       & $\bf 92.24$        & $\bf 93.40$       & $92.15$        & $92.97$        & $90.81$        & $92.65$       & $89.67$        & $90.97$        & $90.07$          & $91.54$          \\
% % ArBench\textsubscript{Dia-B}          & $85.52$       & $84.88$       & $86.54$        & $85.98$       & $87.82$        & $87.17$       & $87.74$        & $87.21$        & $88.31$        & $87.74$       & $88.72$        & $88.19$        & $\bf 88.47$          & $\bf 87.87$          \\
% % ArBench\textsubscript{Dia-R}          & $86.45$       & $85.89$       & $86.00$        & $85.46$       & $86.97$        & $86.54$       & $87.30$        & $86.92$        & $88.85$        & $88.49$       & $\bf 90.94$        & $\bf 90.65$        &$90.04$&	$89.67$            \\
% % ArBench\textsubscript{Dia-C}         & $42.80$       & $35.23$       & $42.67$        & $35.40$       & $41.94$        & $34.98$       & $\bf 39.71$        & $33.56$        & $44.44$        & $36.87$       & $45.89$        & $37.69$        & $\bf 47.49$          & $38.53$          \\
% % ArBench\textsubscript{NER}             & $95.90$       & $69.06$       & $96.02$       & $73.27$       & $96.13$        & $\bf 74.94$       & $96.76$        & $76.19$        & $97.00$        & $76.83$       & $96.38$        & $71.93$        & $\bf 96.75$          & $74.70$          \\
% % ArBench\textsubscript{QA}              & $34.34$       & $55.74$       & $34.62$        & $56.67$       & $39.37$        & $\bf 63.12$       & $36.31$        & $58.10$        & $36.29$        & $57.81$       & $29.13$        & $48.83$        & $\bf 40.47$          & $62.09$          \\
% % ArBench\textsubscript{SM}\textsuperscript{$\ddagger$}              & $77.76$       & $69.88$       & $79.81$        & $71.19$       & $80.01$        & $73.00$       & $78.84$        & $72.03$        & $80.39$        & $74.22$       & $82.35$        & $77.13$       & $0.00$           & $0.00$           \\
% % \toprule
% % \textbf{ArBench\textsubscript{Score}}  & $74.08$       & $71.54$       & $76.09$        & $74.10$       &$77.21$        & $75.89$       & $74.63$        & $73.19$        & $76.76$        & $75.39$       & $77.05$        & $74.92$        & $0$          & $00$    \\
% % \toprule
% % \end{tabular}%
% % }
% % \caption{\small{Performance of our models on ArBench. $^*$~Metric for ArBench\textsubscript{QA} is exact match (EM).$^\dagger$ Metric for ArBench\textsubscript{Senti} is F\textsubscript{1}\textsuperscript{PN}. $^\ddagger$ ArBench\textsubscript{SM} results is the average score across the social meaning tasks described in Table~\ref{tab:SM_res}.}}
% % % \label{tab:NER_res}
% % \end{table*}

% % \begin{table}[t]
% % \centering
% % \footnotesize
% % \begin{adjustbox}{width=0.9\columnwidth}
% % \begin{tabular}{lHHHlHHcc}
% % \toprule
 
% %               &       &      & \multicolumn{1}{c}{} & \multicolumn{2}{l}{~~~~\textbf{}} & \multicolumn{2}{l}{\textbf{~~~~~~~~~~~~~TEST}} \\ 
               
% %               \cline{8-9} 
 
% % %   
% % \multirow{-2}{*}{\textbf{Dataset (classes)}} &    & \multirow{-2}{*}{\textbf{SOTA}}& \multirow{-2}{*}{\textbf{Metric}} & \multirow{-2}{*}{\textbf{LM}}& \textbf{Acc.}              & \textbf{F$_1$}& \textbf{Acc/EM$^*$}            & \textbf{F\textsubscript{1}\textsuperscript{\textit{PN}}/F\textsubscript{1}\textsuperscript{\textit{$\dagger$}}} \\ \toprule



% %  &       &       &    & mBERT             & $0$       &$0$       & $79.02$       & $75.50$       \\
% %  &       &       &    & XLM-R\textsubscript{B}  & $0$       &$0$       & $92.17$       &  $93.00$       \\
% %  &       &       &    & XLM-R\textsubscript{L} & $0$       &$0$      & $93.18$    & \textbf{$\textbf{94.00}$ }   \\
% %  &       &       &    & AraBERT           & $0$       &$0$        & $78.26$      & $78.50$      \\\cdashline{5-9}
% %  &       &       &    & \ourmodel         & $0$       &$0$  & $87.96$ & $88.50$ \\
% %  \multirow{-6}{*}{ArBench\textsubscript{Senti}\textsuperscript{\textit{}}}  &          & \multirow{-6}{*}{} & \multirow{-6}{*}{F1} & \newmodel           & -- & -- & $93.30$ & \textbf{$\textbf{94.00}$}\\\hline 





% % % ############################# 



% %  &       &       &    & mBERT             & $91.1 $&$ 91.67$&$90.88$&$92.12$    \\
% %  &       &       &    & XLM-R\textsubscript{B}  & $91.57 $&$ 92.24$&$90.9$&$91.81$     \\
% %  &       &       &    & XLM-R\textsubscript{L} & $92.66 $&$ \textbf{93.53}$&$92.24$&$\textbf{93.40}$     \\
% %  &       &       &    & AraBERT           & $92.42 $&$ 93.17$&$92.15$&$92.97$     \\\cdashline{5-9}
% %  &       &       &    & \ourmodel         & $91.06 $&$ 92.23$&$90.81$&$92.65$ \\
% % \multirow{-6}{*}{ArBench\textsubscript{Topic}}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{}  & \multirow{-6}{*}{F1} & \newmodel           & $90.48 $&$ 92.01$&$89.67$&$90.97$ \\\hline

% % % 
% % % 
% % % 
% % % 
% % % 
% % % $91.52 $&$ 92.5$&$90.66$&$91.84$

% % % ############################# 



% %  &       &       &    & mBERT             & $87.83$	&$87.50$&	$85.52$&	$84.88$       \\
% %  &       &       &    & XLM-R\textsubscript{B}  &$88.20$&	$87.93$&	$86.54$	&$85.98$      \\
% %  &       &       &    & XLM-R\textsubscript{L} & $88.92$&	$88.57$&	$87.82$	&$87.17$     \\
% %  &       &       &    & AraBERT           &$89.30$&	$89.06$&	$87.74$	&$87.21$        \\\cdashline{5-9}
% %  &       &       &    & \ourmodel         & $89.53$	&$89.23$&	$88.31$	&$87.74$               \\
% % \multirow{-6}{*}{ArBench\textsubscript{Dia-B}}  & \multirow{-6}{*}{---}              &
% % \multirow{-6}{*}{}  & \multirow{-6}{*}{F1} & \newmodel           & $89.80$&	$\textbf{89.50}$&	$88.72$&	$\textbf{88.19}$ \\\hline 
% % % ############################# 

% %  &       &       &    & mBERT             & $86.45$	&$85.89$	&$86.45$	&$85.89$       \\
% %  &       &       &    & XLM-R\textsubscript{B}  & $86.00$&	$85.46$&	$86.00$&	$85.46$        \\
% %  &       &       &    & XLM-R\textsubscript{L} & $86.97$&	$86.54$&	$86.97$&	$86.54$     \\
% %  &       &       &    & AraBERT           & $87.30$&	$86.92$&	$87.30$	&$86.92$        \\\cdashline{5-9}
% %  &       &       &    & \ourmodel         & $88.85$&	$88.49$	&$88.85$&	$88.49$       \\
% % \multirow{-6}{*}{ArBench\textsubscript{Dia-R}}  & \multirow{-6}{*}{---}              &
% % \multirow{-6}{*}{}  & \multirow{-6}{*}{F1} & \newmodel           & $90.94$&	$\textbf{90.65}$&	$90.94$&$\textbf{90.65}$ \\\hline

% % % ############################# 

% %  &       &       &    & mBERT             &$41.08$&	$32.03$	&$42.80$&$35.23$        \\
% %  &       &       &    & XLM-R\textsubscript{B}  & $40.59$&	$31.75$&	$42.67$&	$35.40$       \\
% %  &       &       &    & XLM-R\textsubscript{L} & $39.73$&	$31.51$&	$41.94$&	$34.98$      \\
% %  &       &       &    & AraBERT           & $37.90$	&$30.41$&	$39.71$	&$33.56$       \\
% %  \cdashline{5-9}
% %  &       &       &    & \ourmodel         & $42.51$	&$\textbf{34.26}$&	$44.44$	&$36.87$        \\
 

 
% %  \multirow{-6}{*}{ArBench\textsubscript{Dia-C}}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{}  & \multirow{-6}{*}{F1} & \newmodel         &   $43.54$	&$34.25$&	$45.89$	&$\textbf{37.69}$ \\\hline
% %  % ############################# NER
 
 
% %  &       &       &    & mBERT             & $96.81$	&$76.91$&	$95.90$&	$69.06$       \\
% %  &       &       &    & XLM-R\textsubscript{B}  & $97.74$&	$84.09$	&$96.02$&	$73.27$      \\
% %  &       &       &    & XLM-R\textsubscript{L} & $97.97$	&$85.56$	&$96.13$&	$74.94$     \\
% %  &       &       &    & AraBERT           &     $97.79$	&$\textbf{83.67}$&	$96.76$&	$76.19$  \\\cdashline{5-9}
% %  &       &       &    & \ourmodel         & $97.46$&	$81.21$	&$97.00$&	$\textbf{76.83}$ \\

% %  \multirow{-6}{*}{ArBench\textsubscript{NER}}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{}  & \multirow{-6}{*}{F1} & 
% % \newmodel           & $96.89$	&$76.58$&	$96.38$&	$71.93$ \\\hline

% % % ############################# POS

% % %  &       &       &    & mBERT             &$91.48$	& $89.52$& 	$91.43$	& $89.57$      \\

% % %  &       &       &    & XLM-R\textsubscript{B}  &  $94.02$&	$92.78$	&$94.18$&	$93.04$       \\
% % %  &       &       &    & XLM-R\textsubscript{L} & $95.39$	&$\bf94.47$&	$95.68$	&$\bf94.81$     \\
 
% % %  &       &       &    & AraBERT           & $88.23$& 	$88.26$& 	$88.90$	& $88.87$       \\
 
% % % \cdashline{5-9}
% % %  &       &       &    & \ourmodel         & $91.41$	& $89.48$& 	$91.25$	& $89.28$
% % %         \\
% % % \multirow{-6}{*}{ArBench\textsubscript{POS}}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{}  & \multirow{-6}{*}{F1} & \newmodel        &  $91.29$	& $89.54$& 	$91.45$	& $89.66$  \\\hline 
% % % % \cline{8-9} 

% % % ######################

% % % 

% % %  &    &   & & &        &   & \textbf{EM}              & \textbf{F$_1$} \\ \cline{8-9} 
% %  &       &       &    & mBERT             &   --   &--     & $34.34$&	$55.74$        \\
% %  &       &       &    & XLM-R\textsubscript{B}  &      -- &  --    & $34.62$   &   	$56.67$    \\
% %  &       &       &    & XLM-R\textsubscript{L} & --       &--      & $39.37$       & $\bf63.12$      \\
% %  &       &       &    & AraBERT           & --       &--      &$36.31$&	$58.10$        \\\cdashline{5-9}
% %  &       &       &    & \ourmodel     &    --      &--     & $36.29$	&$57.81$       \\
% %   &       &       &    & \newmodel         & --       &--      & $29.13$	&$48.83$      \\
% %  \multirow{-6}{*}{ArBench\textsubscript{QA}\textsuperscript{\textit{}}}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{}  & \multirow{-6}{*}{F1} & \newmodel~(v2)         & --       &--      & $40.47$&	$62.09$\\\hline 



	



% %  &       &       &    & mBERT             & $76.39$&	$70.59$	&$77.76$&	$69.88$       \\
% %  &       &       &    & XLM-R\textsubscript{B}  & $79.07$&	$73.28$	&$79.81$&	$71.19$       \\
% %  &       &       &    & XLM-R\textsubscript{L} & $78.61$ &	$73.37$ &	$80.01$	& $73.00$      \\
% %  &       &       &    & AraBERT           &$77.29$ &	$70.99$&	$78.84$&	$72.03$        \\\cdashline{5-9}
% %  &       &       &    & \ourmodel     &    $78.99$	&$\bf73.40$&	$80.39$&	$74.22$       \\
% %  \multirow{-6}{*}{ArBench\textsubscript{SM}\textsuperscript{$\ddagger$}}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{}  & \multirow{-6}{*}{F1} & \newmodel         & $81.87$&	$78.15$	&$82.35$&	$\bf77.13$ \\
% %  \toprule
% %   &       &       &    & mBERT             & $0$       &$0$      & $0$       & $0$        \\
% %  &       &       &    & XLM-R\textsubscript{B}  & $0$       &$0$      & $0$       & $0$        \\
% %  &       &       &    & XLM-R\textsubscript{L} & $0$       &$0$      & $0$       & $0$      \\
% %  &       &       &    & AraBERT           & $0$       &$0$      & $0$       & $0$        \\\cdashline{5-9}
% %  &       &       &    & \ourmodel     &    $0$       &$0$      & $0$       & $0$       \\
% %  \multirow{-6}{*}{\textbf{ArBench\textsubscript{Score}}\textsuperscript{\textit{}}}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{}  & \multirow{-6}{*}{F1} & \newmodel         & $0$       &$0$      & $0$       & $0$ \\\hline
 
% % \toprule

% % \end{tabular}
% % \end{adjustbox}
% % \caption{\small{Performance of our models on ArBench. $^*$Metric for ArBench\textsubscript{QA} is exact match (EM).$^\dagger$ Metric for ArBench\textsubscript{Senti} is F\textsubscript{1}\textsuperscript{PN}. $^\ddagger$ ArBench\textsubscript{SM} results is the average score across the social meaning tasks described in Table~\ref{tab:SM_res}.}}
% % \label{tab:NER_res}
% % \end{table}

==> tables/MT_Res_X_AR_TEST.tex <==


\begin{table}[t]
\centering
 \renewcommand{\arraystretch}{1.3}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule 
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{S/M}} & \multicolumn{2}{c}{\textbf{DEV}}              & \multicolumn{2}{c}{\textbf{TEST}} \\ \cline{3-6}
                      &                                    & \multicolumn{1}{c}{\textbf{mT5}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{mT5}    & \textbf{AraT5\textsubscript{MSA}}     \\ 
% \textbf{Dataset}     & \textbf{S/M} & \textbf{mT5} & \textbf{AraT5\textsubscript{MSA}} & \textbf{mT5} & \textbf{AraT5\textsubscript{MSA}}  \\
% \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{Acc/EM}                       & \textbf{FPN/F1}                      & \textbf{Acc/EM}             & \textbf{FPN/F1}            & \textbf{Acc/EM}                 & \textbf{FPN/F1}                 & \textbf{Acc/EM}                & \textbf{FPN/F1}               & \textbf{Acc/EM}                   & \textbf{FPN/F1}                 \\
\toprule 
\multicolumn{1}{c}{\multirow{2}{*}{DE \rightarrow AR}}
  & S                              & $12.88$&$\bf13.74$&$11.92$&$\bf12.80$\\
  & M                                 & $\bf16.49$&$15.83$&$\bf15.35$&$14.68$\\   \hline
\multicolumn{1}{c}{\multirow{2}{*}{FR \rightarrow AR }}                                       & S       &  $17.52$&$\bf17.96$&$18.61$&$\bf18.99$\\ 
& M                               & $19.49$&$\bf19.55$&$\bf21.05$&$20.98$\\     \hline
\multicolumn{1}{c}{\multirow{2}{*}{RU \rightarrow AR}}                                     & S                                & $26.78$&$\bf27.87$&$26.63$&$\bf28.01$\\       
  & M                              & $27.41$&$\bf27.75$&$27.20$&$\bf28.05$\\      \toprule
\multicolumn{1}{c}{\multirow{2}{*}{HI \rightarrow AR}}                                     & S                 & $\bf04.68$&$01.78$&$\bf04.85$&$02.00$\\       
  & M                                & $\bbf04.19$&$02.82$&$\bf04.62$&$03.23$\\       \hline
\multicolumn{1}{c}{\multirow{2}{*}{IG \rightarrow AR}}                                     & S                                & $\bf02.04$&$00.65$&$\bf02.71$&$00.62$\\            
  & M                                &  $\bf14.044$&$09.60$&$\bf19.61$&$14.61$\\        \hline
\multicolumn{1}{c}{\multirow{2}{*}{YO \rightarrow AR}}                                     & S                                & $\bf01.26$&$00.589$&$\bf01.40$&$01.23$\\  
  & M                                &  $\bf21.23$&$17.14$&$\bf21.39$&$17.25$\\
    \toprule             
\end{tabular}%
}
\caption{\hl{Performance of our models on X to AR ARGEN\textsubscript{CS} development and test datasets on single (\textbf{S}) and multi-tasks (\textbf{M}) setting in BLEU. \textbf{FR:} French, \textbf{DE:} German, \textbf{RU:}  Russian, \textbf{HI:} Hindi, \textbf{YO:} Yoruba, \textbf{IG:} Igbo. }}  \label{tab:x_to_ar_res}
\end{table}







==> tables/MT_Res_X_AR_TEST_in_out_voacab.tex <==
\begin{table}[t]
\centering
 \renewcommand{\arraystretch}{1.3}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{lHcccc}
\toprule 
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{S/M}} & \multicolumn{2}{c}{\textbf{DEV}}              & \multicolumn{2}{c}{\textbf{TEST}} \\ \cline{3-6}
                      &                                    & \multicolumn{1}{c}{\textbf{mT5}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{mT5}    & \textbf{AraT5\textsubscript{MSA}}     \\ 
% \textbf{Dataset}     & \textbf{S/M} & \textbf{mT5} & \textbf{AraT5\textsubscript{MSA}} & \textbf{mT5} & \textbf{AraT5\textsubscript{MSA}}  \\
% \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{Acc/EM}                       & \textbf{FPN/F1}                      & \textbf{Acc/EM}             & \textbf{FPN/F1}            & \textbf{Acc/EM}                 & \textbf{FPN/F1}                 & \textbf{Acc/EM}                & \textbf{FPN/F1}               & \textbf{Acc/EM}                   & \textbf{FPN/F1}                 \\
\toprule 
\multicolumn{1}{c}{\multirow{1}{*}{DE \rightarrow AR}}
   & S                         &  0.999&0.018&0.556&0.016\\
%   & M                                 & $\bf16.49$&$15.83$&$\bf15.35$&$14.68$\\   \hline
\multicolumn{1}{c}{\multirow{1}{*}{FR \rightarrow AR }}                                      & S                              & 0.874&0.028&0.769&0.019\\
% & M                               & $19.49$&$\bf19.55$&$\bf21.05$&$20.98$\\     \hline
\multicolumn{1}{c}{\multirow{1}{*}{RU \rightarrow AR}}                               & S                              & 1.161&0.139&0.532&0.137\\
%   & M                              & $27.41$&$\bf27.75$&$27.20$&$\bf28.05$\\      
\toprule
\multicolumn{1}{c}{\multirow{1}{*}{HI \rightarrow AR}}                                     & S                  & 0.188&0.014&0.036&0.016\\    
%   & M                                & $\bbf04.19$&$02.82$&$\bf04.62$&$03.23$\\       \hline
\multicolumn{1}{c}{\multirow{1}{*}{IG \rightarrow AR}}                                     & S                            &     3.988&0.269&6.095&0.131\\            
%   & M                                &  $\bf14.044$&$09.60$&$\bf19.61$&$14.61$\\        \hline
\multicolumn{1}{c}{\multirow{1}{*}{YO \rightarrow AR}}                                     & S                           &    3.340&0.007&6.784&0.005\\ 
%   & M                                &  $\bf21.23$&$17.14$&$\bf21.39$&$17.25$\\
    \toprule             
\end{tabular}%
}
\caption{\hl{Performance of our models train on 1K X-AR sentences on  ARGEN\textsubscript{CS} development and test datasets in BLEU. \textbf{FR:} French, \textbf{DE:} German, \textbf{RU:}  Russian, \textbf{HI:} Hindi, \textbf{YO:} Yoruba, \textbf{IG:} Igbo.} }  \label{tab:x_to_ar_res_in_out_vocab}
\end{table}




% \begin{table}[t]
% \centering
%  \renewcommand{\arraystretch}{1.3}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{lccccc}
% \toprule 
% \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{S/M}} & \multicolumn{2}{c}{\textbf{DEV}}              & \multicolumn{2}{c}{\textbf{TEST}} \\ \cline{3-6}
%                       &                                    & \multicolumn{1}{c}{\textbf{mT5}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{mT5}    & \textbf{AraT5\textsubscript{MSA}}     \\ 
% % \textbf{Dataset}     & \textbf{S/M} & \textbf{mT5} & \textbf{AraT5\textsubscript{MSA}} & \textbf{mT5} & \textbf{AraT5\textsubscript{MSA}}  \\
% % \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{Acc/EM}                       & \textbf{FPN/F1}                      & \textbf{Acc/EM}             & \textbf{FPN/F1}            & \textbf{Acc/EM}                 & \textbf{FPN/F1}                 & \textbf{Acc/EM}                & \textbf{FPN/F1}               & \textbf{Acc/EM}                   & \textbf{FPN/F1}                 \\
% \toprule 
% \multicolumn{1}{c}{\multirow{2}{*}{DE \rightarrow AR}}
%   & S                              & $12.88$&$\bf13.74$&$11.92$&$\bf12.80$\\
%   & M                                 & $\bf16.49$&$15.83$&$\bf15.35$&$14.68$\\   \hline
% \multicolumn{1}{c}{\multirow{2}{*}{FR \rightarrow AR }}                                       & S       &  $17.52$&$\bf17.96$&$18.61$&$\bf18.99$\\ 
% & M                               & $19.49$&$\bf19.55$&$\bf21.05$&$20.98$\\     \hline
% \multicolumn{1}{c}{\multirow{2}{*}{RU \rightarrow AR}}                                     & S                                & $26.78$&$\bf27.87$&$26.63$&$\bf28.01$\\       
%   & M                              & $27.41$&$\bf27.75$&$27.20$&$\bf28.05$\\      \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{HI \rightarrow AR}}                                     & S                 & $\bf04.68$&$01.78$&$\bf04.85$&$02.00$\\       
%   & M                                & $\bbf04.19$&$02.82$&$\bf04.62$&$03.23$\\       \hline
% \multicolumn{1}{c}{\multirow{2}{*}{IG \rightarrow AR}}                                     & S                                & $\bf02.04$&$00.65$&$\bf02.71$&$00.62$\\            
%   & M                                &  $\bf14.044$&$09.60$&$\bf19.61$&$14.61$\\        \hline
% \multicolumn{1}{c}{\multirow{2}{*}{YO \rightarrow AR}}                                     & S                                & $\bf01.26$&$00.589$&$\bf01.40$&$01.23$\\  
%   & M                                &  $\bf21.23$&$17.14$&$\bf21.39$&$17.25$\\
%     \toprule             
% \end{tabular}%
% }
% \caption{Performance of our models on X to AR ARGEN\textsubscript{CS} development and test datasets on single (\textbf{S}) and multi-tasks (\textbf{M}) setting in BLEU. \textbf{FR:} French, \textbf{DE:} German, \textbf{RU:}  Russian, \textbf{HI:} Hindi, \textbf{YO:} Yoruba, \textbf{IG:} Igbo. }  \label{tab:x_to_ar_res}
% \end{table}

















% \begin{table}[t]
% \centering
%  \renewcommand{\arraystretch}{1.2}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{lccccc}
% \toprule 
% \textbf{Dataset}     & \textbf{S/M} & \textbf{mT5} & \textbf{AraT5\textsubscript{Tweet}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{AraT5} \\
% % \multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{Acc/EM}                       & \textbf{FPN/F1}                      & \textbf{Acc/EM}             & \textbf{FPN/F1}            & \textbf{Acc/EM}                 & \textbf{FPN/F1}                 & \textbf{Acc/EM}                & \textbf{FPN/F1}               & \textbf{Acc/EM}                   & \textbf{FPN/F1}                 \\
% \toprule 
% \multicolumn{1}{c}{\multirow{2}{*}{FR \rightarrow AR}}
%   & S                              & $\bfxx$	& $xx$	& $18.99$	& $xx$      \\   
%   & M                                 & $\bfxx$	& $xx$	& $20.98$	& $xx$      \\   \hline
% \multicolumn{1}{c}{\multirow{2}{*}{DE \rightarrow AR }}                                       & S       &  xx &xx &  $12.79$ & xx \\
% & M                               & $\bfxx$	& $xx$	& $14.68$ 	& $xx$     \\   \hline
% \multicolumn{1}{c}{\multirow{2}{*}{RU \rightarrow AR}}                                     & S                                & $\bfxx$	& $xx$	& $28.01$	& $xx$      \\  
%   & M                              & $\bfxx$	& $xx$	& $28.04$	& $xx$      \\   \hline \hline
% \multicolumn{1}{c}{\multirow{2}{*}{HI \rightarrow AR}}                                     & S                 & $\bfxx$	& $xx$	& $2.01$	& $xx$      \\   
%   & M                                & $\bfxx$	& $xx$	& $xx$	& $xx$      \\   \hline
% \multicolumn{1}{c}{\multirow{2}{*}{IG \rightarrow AR}}                                     & S                                & $\bfxx$	& $xx$	& $0.62$	& $xx$                        \\  
%   & M                                &  $\bf19.15$	& $xx$	& $11.14$	& $xx$         \\ \hline
% \multicolumn{1}{c}{\multirow{2}{*}{YO \rightarrow AR}}                                     & S                                &  $\bfxx$	& $xx$	& $1.40$	& $xx$            \\  
%   & M                                &  $\bf19.63$	& $xx$	& $13.44$	& $xx$                        \\  
%     \toprule             
% \end{tabular}%
% }
% \caption{Performance of our models on X to AR ARGEN\textsubscript{CS} TEST datasets on single and multi tasks setting in BLEU. \textbf{FR:} French, \textbf{DE:} German, \textbf{RU:}  Russian, \textbf{HI:} Hindi, \textbf{YO:} Yoruba, \textbf{IG:} Igbo. }  \label{tab:x_to_ar_res}
% \end{table}

==> tables/MT_Results_Arabic_to_Eng.tex <==
\begin{table*}[t]
\centering
\footnotesize
 \renewcommand{\arraystretch}{1.25}
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{lllHrrrrrr|r}
\toprule
\multicolumn{2}{c}{ \textbf{\footnotesize Dataset}   }    & \textbf{\footnotesize Test Split}  & \textbf{\footnotesize SOTA}    & \textbf{S2S\textsubscript{2M}}  & \textbf{S2S\textsubscript{10M}}&  \textbf{ \footnotesize mT5}  & \textbf{\footnotesize AraT5\textsubscript{Tweet}} & \textbf{ \footnotesize AraT5\textsubscript{MSA}} & \textbf{ \footnotesize AraT5\textsubscript{}}  & \textbf{\footnotesize SOTA}\\

\multicolumn{2}{c}{  }    &  AR$\leftrightarrow$EN  & \textbf{\footnotesize SOTA}    &  $\rightarrow$ $\leftarrow$    & $\rightarrow$ $\leftarrow$&  $\rightarrow$ $\leftarrow$ & $\rightarrow$ $\leftarrow$& $\rightarrow$ $\leftarrow$ & $\rightarrow$ $\leftarrow$ & $\rightarrow$ $\leftarrow$\\
\toprule

&\multirow{2}{*}{{\textbf{ADPT}}\textsuperscript{$\dagger$} }   &  Lev &  $\bf10.80$   /  **.** &    $4.30$   /  **.** &    $6.20$   /  **.** &    $8.33$   /  **.** &    $8.32$   /  **.** &    $\bf8.52$   /  **.** &    $8.42$ /  **.**  &  $10.80$     \\
&    &  Egy   &  $\bf14.00$ /  **.** & $5.21$/  **.**&$8.9$ /  **.** & $12.57$ /  **.** & $11.25$ /  **.** & $12.38$ /  **.** & $\bf12.92$ /  **.** &   $14.00$   \\
\cdashline{2-11}
&\multirow{2}{*}{{\textbf{Bible I}\textsuperscript{$\dagger$}} }  & \multirow{1}{*}{Tun.}     & $7.00$   /  **.** &    $4.12$   /  **.** &    $4.44$   /  **.** &    $8.08$   /  **.** &    $5.86$   /  **.** &    $\bf8.52$   /  **.** &    $7.94$ /  **.**  &  $7.00$         \\
 & &     \multirow{1}{*}{Mor.}      &$4.20$   /  **.** &    $2.60$   /  **.** &    $2.80$   /  **.** &    $7.21$   /  **.** &    $4.69$   /  **.** &    $\bf7.83$   /  **.** &    $6.82$   /  **.** &    $4.20$          \\ \cdashline{2-11}






& \multirow{5}{*}{\textbf{MADAR I}\textsuperscript{$\dagger$}}  & \multirow{1}{*}{Egy.} &$\bf28.90$   /  **.** &    $17.25$   /  **.** &    $17.71$   /  **.** &    $24.44$   /  **.** &    $21.75$   /  **.** &    $\bf24.98$   /  **.** &    $24.66$ /  **.**  &  $28.90$   \\
& & \multirow{1}{*}{{Qat.}}                                   &$\bf27.60$   /  **.** &    $15.98$   /  **.** &    $17.92$   /  **.** &    $23.72$   /  **.** &    $22.23$   /  **.** &    $\bf24.00$   /  **.** &    $23.92$   /  **.** &    $27.60$   \\  
& &\multirow{1}{*}{{Leb.}}                                      & $\bf17.00$   /  **.** &    $12.15$   /  **.** &    $10.14$   /  **.** &    $14.6$   /  **.** &    $12.25$   /  **.** &    $\bf14.92$   /  **.** &    $14.18$  /  **.**  & $17.00$\\ 
& &\multirow{1}{*}{{Tun.}}                                        & $\bf11.40$   /  **.** &    $8.49$   /  **.** &    $8.57$   /  **.** &    $10.12$   /  **.** &    $9.09$   /  **.** &    $\bf10.18$   /  **.** &    $9.60$  /  **.**  & $11.40$    \\  
& &\multirow{1}{*}{{Mor.}}                                        & $\bf14.70$   /  **.** &    $11.07$   /  **.** &    $11.83$   /  **.** &    $16.61$   /  **.** &    $12.37$   /  **.** &    $\bf16.99$   /  **.** &    $16.82$ /  **.**  & $14.70$  \\   \cdashline{2-11}





\multirow{18}{*}{{\textbf{DIA}}}  &\multirow{20}{*}{{\textbf{MADAR II}\textsuperscript{$\dagger$}} } 
& Egy-Alex.   &  $28.90$   /  **.** &    $19.01$   /  **.** &    $19.74$   /  **.** &    $29.34$   /  **.** &    $24.79$   /  **.** &    $\bf29.87$   /  **.** &    $29.02$  /  **.**  &  $28.90$   \\
& &  Egy-Asw.  & $\bf26.30$   /  **.** &    $16.37$   /  **.** &    $16.95$   /  **.** &    $23.01$   /  **.** &    $19.52$   /  **.** &    $\bf23.41$   /  **.** &    $22.06$ /  **.**  & $26.30$\\
& &  Sud-Kha.  &$\bf36.70$   /  **.** &    $24.97$   /  **.** &    $25.65$   /  **.** &    $30.87$   /  **.** &    $28.13$   /  **.** &    $\bf31.39$   /  **.** &    $30.65$      /  **.**  & $36.70$       \\ 
% & &  Qat-Doha  &  - &- & - & -   &      -   &  -          \\
& &  Yem-San.  & $\bf29.90$   /  **.** &    $19.62$   /  **.** &    $20.35$   /  **.** &    $24.87$   /  **.** &    $23.19$   /  **.** &    $\bf26.10$   /  **.** &    $25.73$    /  **.**  &  $29.90$     \\
& &  Oma-Mus. & $\bf39.50$   /  **.** &    $29.12$   /  **.** &    $30.66$   /  **.** &    $33.74$   /  **.** &    $32.15$   /  **.** &    $\bf34.62$   /  **.** &    $34.18$  /  **.**  &  $39.50$      \\
& &  KSA-Riy. &  $\bf40.70$   /  **.** &    $26.14$   /  **.** &    $26.66$   /  **.** &    $33.54$   /  **.** &    $30.81$   /  **.** &    $\bf33.86$   /  **.** &    $33.59$   /  **.**  & $40.70$    \\
& &  KSA-Jed. & $\bf27.40$   /  **.** &    $16.08$   /  **.** &    $17.21$   /  **.** &    $\bf23.57$   /  **.** &    $20.91$   /  **.** &    $23.45$   /  **.** &    $23.11$  /  **.**  & $27.40$      \\
& &  Iraq-Bag. & $\bf28.30$   /  **.** &    $15.98$   /  **.** &    $19.09$   /  **.** &    $22.92$   /  **.** &    $20.84$   /  **.** &    $23.24$   /  **.** &    $\bf22.52$ /  **.**  &  $28.30$     \\ 
& &  Iraq-Bas. & $\bf27.70$   /  **.** &    $16.46$   /  **.** &    $17.12$   /  **.** &    $\bf22.94$   /  **.** &    $20.47$   /  **.** &    $22.61$   /  **.** &    $22.00$  /  **.**  & $27.70$    \\ 
& &  Iraq-Mos.  & $\bf30.00$   /  **.** &    $18.25$   /  **.** &    $19.14$   /  **.** &    $23.69$   /  **.** &    $21.95$   /  **.** &    $\bf24.41$   /  **.** &    $23.12$  /  **.**  & $30.00$      \\ 

% & & Leb-Bei. &  - &- &  - & - &    - & -          \\
& & Pal-Jer. &  $\bf27.0$   /  **.** &    $15.18$   /  **.** &    $16.06$   /  **.** &    $24.61$   /  **.** &    $20.91$   /  **.** &    $\bf24.95$   /  **.** &    $24.45$   /  **.**  &  $27.0$ \\
& & Jor-Amm. &  $\bf30.00$   /  **.** &    $18.68$   /  **.** &    $18.86$   /  **.** &    $26.45$   /  **.** &    $22.92$   /  **.** &    $\bf26.78$   /  **.** &    $25.26$     /  **.**  &  $30.00$   \\
& & Jor-Salt. & $\bf29.60$   /  **.** &    $17.14$   /  **.** &    $17.78$   /  **.** &    $26.04$   /  **.** &    $23.05$   /  **.** &    $\bf26.56$   /  **.** &    $26.05$   /  **.**  & $29.60$  \\
& &  Syr-Dam. &  $\bf25.90$   /  **.** &    $13.63$   /  **.** &    $14.83$   /  **.** &    $21.93$   /  **.** &    $18.55$   /  **.** &    $\bf22.54$   /  **.** &    $21.80$   /  **.**  &  $25.90$   \\
& &  Syr-Alep. &  $\bf26.40$   /  **.** &    $14.16$   /  **.** &    $15.27$   /  **.** &    $22.39$   /  **.** &    $19.55$   /  **.** &    $22.91$   /  **.** &    $\bf23.26$   /  **.**  &  $26.40$  \\  
& &   Alg-Alg.  & $\bf17.30$   /  **.** &    $13.94$   /  **.** &    $14.24$   /  **.** &    $16.97$   /  **.** &    $14.26$   /  **.** &    $\bf17.46$   /  **.** &    $16.62$   /  **.**  & $17.30$\\ 
& &  Lyb-Trip. & $\bf22.80$   /  **.** &    $14.49$   /  **.** &    $15.44$   /  **.** &    $20.1$   /  **.** &    $17.56$   /  **.** &    $\bf20.31$   /  **.** &    $19.85$  /  **.**  & $22.80$  \\ 
& &  Lyb-Beng. & $\bf28.40$   /  **.** &    $19.02$   /  **.** &    $19.32$   /  **.** &    $25.5$   /  **.** &    $23.39$   /  **.** &    $25.46$   /  **.** &    $\bf25.50$ /  **.**  & $28.40$ \\ 
& &   Tun-Saf & $\bf10.80$   /  **.** &    $7.89$   /  **.** &    $8.57$   /  **.** &    $9.26$   /  **.** &    $8.15$   /  **.** &    $\bf9.94$   /  **.** &    $9.60$     /  **.**  & $10.80$ \\ 
% & &   Tun-Saf & - & - &    &    - & -   &      -    \\ 
% & &  Mor-Fes &  - &- &    &      - & -   &    -    \\ 
& &  Mor-Fes & $20.90$   /  **.** &    $15.09$   /  **.** &    $15.59$   /  **.** &    $22.81$   /  **.** &    $17.33$   /  **.** &    $\bf23.33$   /  **.** &    $21.97$   /  **.** &  $20.90$ \\ \cdashline{2-11}
&\textbf{QAraC}\textsuperscript{$\dagger$} & Qatar & $\bf11.9$   /  **.** &    $10.33$   /  **.** &    $10.47$   /  **.** &    $\bf11.84$   /  **.** &    $11.11$   /  **.** &    $11.42$   /  **.** &    $10.57$   /  **.**  & $11.9$ \\ 
\toprule
\multirow{6}{*}{{\textbf{MSA}}}  & \multirow{2}{*}{{\textbf{Bible II}\textsuperscript{$\dagger$}}}  &  Test 1   &$\bf17.00$   /  **.** &    $10.44$   /  **.** &    $10.86$   /  **.** &    $15.58$   /  **.** &    $13.04$   /  **.** &    $\bf16.38$   /  **.** &    $15.71$  /  **.** &  $17.00$   \\
  &   & Test 2   & $\bf12.80$   /  **.** &    $5.55$   /  **.** &    $6.2$   /  **.** &    $12.1$   /  **.** &    $9.2$   /  **.** &    $\bf12.53$   /  **.** &    $11.64$  /  **.**  & $12.80$          \\ \cdashline{2-11}
  & \textbf{MADAR I}\textsuperscript{$\dagger$}   & MSA & $\bf11.90$   /  **.** &    $10.33$   /  **.** &    $10.47$   /  **.** &    $\bf11.84$   /  **.** &    $11.11$   /  **.** &    $11.42$   /  **.** &    $10.57$ /  **.**  & $11.90$    \\   \cdashline{2-11}
  & \multirow{3}{*}{\textbf{IWSLT}\textsuperscript{$\ddagger$}}  &  TED15 &  $\bf34.1$   /  **.** &    $27.6$   /  **.** &    $28.73$   /  **.** &    $29.39$   /  **.** &    $28.2$   /  **.** &    $30.37$   /  **.** &    $\bf30.45$ /  **.** &   $34.1$                \\
  & & TED16  &   $\bf31.80$   /  **.** &    $25.7$   /  **.** &    $25.77$   /  **.** &    $28.39$   /  **.** &    $27.03$   /  **.** &    $\bf29.37$   /  **.** &    $29.18$    /  **.**  &   $31.80$             \\ 
  &  & QED16  &  $\bf28.10$   /  **.** &    $19.44$   /  **.** &    $19.9$   /  **.** &    $\bf21.09$   /  **.** &    $18.55$   /  **.** &    $20.98$   /  **.** &    $19.11$  /  **.**  &  $28.10$              \\ \cdashline{2-10}
   
    & \textbf{UN}\textsuperscript{$\dagger\dagger$} &Ar-En&$\bf56.90$   /  **.** &    $52.54$   /  **.** &    $53.12$   /  **.** &    $52.38$   /  **.** &    $51.48$   /  **.** &    $53.29$   /  **.** &    $\bf52.96$ /  **.**   &$56.90$              \\


\toprule
  &  &    \textbf{\textit{Average}} & $\bf25.75$   /  **.** &    $17.26$   /  **.** &    $17.92$   /  **.** &    $22.47$   /  **.** &    $20.06$   /  **.** &    $\bf22.91$   /  **.** &    $22.31$ /  **.**  &  $25.75$\\
 %  ---------- DIA -----------


 
% \newcite{elmahdy2014development}    & $-$   &   & $-$ &  $14.7$K   \\


\toprule

\end{tabular}}
\caption{Arabic to English results using ARGEN\textsubscript{MT}  datasets. \textbf{S2S:} Sequence-to-Sequence Transformer models trained from scratch on $2$M and $10$M parallel sentences. \textbf{SOTA:} \textsuperscript{$\dagger$}~\newcite{sajjad2020arabench}, \textsuperscript{$\ddagger$}~\newcite{durrani2017qcri}, \textsuperscript{$\dagger\dagger$}~\newcite{junczys2016neural}.}
\label{tab:rs_mt_data}

\end{table*}


==> tables/MT_data.tex <==


\begin{table}[ht]
\centering
 \renewcommand{\arraystretch}{1.1}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{llHHHcc}
\toprule
 \textbf{Variety}   & \textbf{Dataset}        & \textbf{Region}     &  \textbf{Countries}  & \textbf{City}           & \textbf{DEV}            & \textbf{TEST}                  \\
\toprule

\multirow{4}{*}{{\textbf{DIA}}}   &\multirow{2}{*}{{ADPT}~\cite{zbib2012machine} }   &  Lev.  & $-$   &  $-$   & -    &  $138$K    \\
 & &  Nile   &1 &  $-$  & -   & $38$K                   \\   %\cdashline{2-7}
&\multirow{1}{*}{{Bible I}~\cite{sajjad2020arabench}}  & \multirow{1}{*}{Magh.}     &2 & $-$   &  $600$  &   $600$                   \\ %\cdashline{2-7}

&\multirow{1}{*}{{MADAR I }~\cite{bouamor2018madar}  }  & 4 regions & 5   & $-$    &      $5.5$K   &  $6.5$K     \\
% & & \multirow{1}{*}{{Gulf}}   &  1 & -  &     $5.5$K   &  $6.5$K       \\  
% & &\multirow{1}{*}{{Leven.}}  &  1 & -   &    $5.5$K   &  $6.5$K     \\ 
% & &\multirow{1}{*}{{Magh.}}    &  2  & -   &     $5.5$K   &  $6.5$K      \\   \cline{2-7} 

 &\multirow{1}{*}{{MADAR II}~\cite{bouamor2018madar}} & 4 regions & 16  & 21   &     -    &  $2$K     \\
% & & \multirow{1}{*}{{Gulf}}   &  6 & 8   &      -   &  $2K$           \\  
% & &\multirow{1}{*}{{Leven.}}  &  4 & 6   &    -   &     $2K$          \\ 
% & &\multirow{1}{*}{{Magh.}}    &  4  & 7   &      -   &  $2K$       \\    
&\multirow{1}{*}{{QAraC}~\cite{sajjad2020arabench}} & Gulf & 1  & 1   &     $6.7$K    &  $6.7$K     \\


\toprule
\multirow{4}{*}{{\textbf{MSA}}}  & \multirow{1}{*}{{Bible II} \newcite{sajjad2020arabench}}  &  $- $   & $-$  &  $-$   & $600$ & $600$    \\ 
% \cdashline{3-7} 
   & {MADAR II}~\cite{bouamor2018madar}     & $-$   &  $-$ & $-$   & $5.5$K   &     $6.5$K       \\   
%   \cdashline{3-7} 
   & \multirow{1}{*}{{IWSLT }~\cite{cettolo2016iwslt}}  &  $-$  & $-$  &$-$ & $1.1$K  & $1.1$K                   \\
  
%   & &  $-$    & $-$  &  $-$   & $1.1$K &$1.1$K       \\
%                                             &  &  $-$   & $-$ & $-$   & $1.1$K &  $549$ \\ 
% \cdashline{3-7}
                                            
%   & \multirow{2}{*}{{NIST} }  &  $-$  & $-$  &$-$ & $-$   & $1.1$K                   \\
  
%   & &  $-$    & $-$  &  $-$   & $-$  &$1.1$K       \\\cdashline{3-7}
                                          
    &  {UN}~\cite{ziemski2016united} & $-$ & $-$ & $-$ & $4$K &  $4$K      \\      
        &  {OPUS-X-Ara} & $-$ & $-$ & $5$K & $5$K &  $5$K                   \\ 





 %  ---------- DIA -----------


 
% \newcite{elmahdy2014development}    & $-$   &   & $-$ &  $14.7$K   \\


\toprule
% {Total}   & & & & &   \\
% \toprule
\end{tabular}}
\caption{Arabic to English datasets included in ARGEN\textsubscript{MT}.  \textbf{MADAR~I:} corpus consists of 2k sentences (Test) of 21 city-level dialects each.  \textbf{MADAR~II:}  12k sentences (5.5k  for Dev, and 6.5k  for Test sets) each of five other city-level dialects and MSA. \textbf{Bible~I:} $600$ sentences each as Dev and Test sets for Moroccan, Tunisian,  and MSA.\textbf{ Bible~II:} Two  Dev and Test splits ($600$ sentences each) are used for Bible MSA. }
% \textbf{NIST:} 1.1k sentences from OpenMT 2004 and 2005 evaluation datasets. 


\label{tab:mt_data}

\end{table}




% \begin{table*}[ht]
% \centering
%  \renewcommand{\arraystretch}{1}
% \resizebox{1.8\columnwidth}{!}{%
% \begin{tabular}{lllcccc}
% \toprule
%  \textbf{Varieties}   & \textbf{Dataset}        & \textbf{Region}     &  \textbf{\#Countr}  & \textbf{\#City}           & \textbf{Dev}            & \textbf{Test}                  \\
% \toprule

% &\multirow{2}{*}{{ADPT}~\newcite{zbib2012machine} }   &  Leven.  & xx   &  -  & -   &  $138$K    \\
%  & &  Nile   &1 &  - & -  & $38$K                   \\   \cdashline{2-7}
% &\multirow{1}{*}{{Bible}\textsuperscript{$\dagger$} \newcite{sajjad2020arabench}}  & \multirow{1}{*}{Magh.}     &2 &  -  &  $600$  &   $600$                   \\ \cdashline{2-7}

% \multirow{4}{*}{{\textbf{DIA}}}  &\multirow{4}{*}{{MADAR I }~\newcite{bouamor2018madar}  }  & \multirow{1}{*}{Nile}   & 1   & -   &      $5.5$K   &  $6.5$K     \\
% & & \multirow{1}{*}{{Gulf}}   &  1 & -  &     $5.5$K   &  $6.5$K       \\  
% & &\multirow{1}{*}{{Leven.}}  &  1 & -   &    $5.5$K   &  $6.5$K     \\ 
% & &\multirow{1}{*}{{Magh.}}    &  2  & -   &     $5.5$K   &  $6.5$K      \\   \cline{2-7} 

%  &\multirow{4}{*}{{MADAR II}~\newcite{bouamor2018madar}} & \multirow{1}{*}{Nile}   & 2   & 4   &      -   &  $2K$     \\
% & & \multirow{1}{*}{{Gulf}}   &  6 & 8   &      -   &  $2K$           \\  
% & &\multirow{1}{*}{{Leven.}}  &  4 & 6   &    -   &     $2K$          \\ 
% & &\multirow{1}{*}{{Magh.}}    &  4  & 7   &      -   &  $2K$       \\    



% \toprule
% \multirow{6}{*}{{\textbf{MSA}}}  & \multirow{2}{*}{{Bible}\textsuperscript{$\ddagger$} \newcite{sajjad2020arabench}}  &  -    & -  &  -   & $600$ & $600$    \\
%   &   &  -    & -  &  -   & $600$ & $600$    \\
%   & {MADAR I}~\newcite{bouamor2018madar}     & -   &  - & -   & $6.5$K   &     $6.5$K       \\ 
%   & {IWSLT 2015}~\newcite{cettolo2016iwslt} &  -  & -  & -  & -  & -                   \\
%   & {IWSLT 2016}~\newcite{cettolo2016iwslt} &-&  -  & - & -  & -                  \\ 
%     &  {UN} \newcite{ziemski2016united} & - & - & - & $4$K &  $4$K                   \\





%  %  ---------- DIA -----------


 
% % \newcite{elmahdy2014development}    & $-$   &   & $-$ &  $14.7$K   \\


% \toprule
% % {Total}   & & & & &   \\
% % \toprule
% \end{tabular}}
% \caption{Arabic Machine translation datasets included in ARGEN\textsubscript{Trans}.  For  MADAR and Bible datasets we use the same splits used by \newcite{sajjad2020arabench}. \textbf{MADAR I:} corpus consists of 2k sentences (TEST) of 21 city-level dialects each.  \textbf{MADAR II }sentences each of 4  city-level dialects and of MSA. 12k (5.5k sentences for DEV, and 6.5k  for TEST sets) sentences each of 4 other city-level dialects and of MSA. {Bible}\textsuperscript{$\ddagger$} Two Dev and Test  splits (600 sentences each) are used     }
% \label{tab:mt_data}

% \end{table*}


==> tables/X_to_AR_MT_Data_splits.tex <==

\begin{table}[t]
 \centering
 \footnotesize

 \begin{tabular}{lccc}
 \toprule
\textbf{Languages} & \textbf{TRAIN}   &  \textbf{DEV} & \textbf{TEST}\\
\toprule
\textbf{DE-AR}     &    $1M$ & $5K$   &$5K$  \\
\textbf{FR-AR}     &    $1M$ & $5K$   &$5K$  \\
\textbf{RU-AR}     &    $1M$ & $5K$   &$5K$  \\ \hline
\textbf{HI-AR}     &    $300K$ & $5K$   &$5K$  \\
\textbf{IG-AR}     &    $1.6K$ & $100$   &$100$  \\
\textbf{YO-AR}     &  $1.4K$ & $100$   &$100$  \\
\toprule 
\end{tabular}
\caption{X to Arabic Machine translation datasets included in ARGEN\textsubscript{MT}. }  \label{tab:x_to_ar_splits}

    \end{table}

==> tables/seq_length_dev.tex <==

\begin{table}[]
\centering
\resizebox{0.9\columnwidth}{!}{%

\begin{tabular}{lcccc}

\toprule
  \textbf{Dataset}  &  \textbf{mT5} & \textbf{AraT5\textsubscript{Tweet}} & \textbf{AraT5\textsubscript{MSA}} & \textbf{AraT5\textsubscript{}} \\ \hline
    & \multicolumn{4}{c}{All Length}                                                                                                                                                                                                        \\ \hline
MSA & $28.76$                   & $27.09$                         & $\bf29.54$                 & $28.75$                     \\
DA  & $15.81$                   & $14.01$                         & \textbf{$\bf16.05$}                 & $15.07$                     \\
All & $18.59$                   & $16.78$                         & \textbf{$\bf18.99$}                 & $17.93$                     \\\hline
    & \multicolumn{4}{c}{Sequence  length $<$ $10$}                                                                                                                                                                         \\\hline
MSA & $38.79$                   & $38.04$                         & \textbf{$\bf39.8$}                  & $38.94$                     \\
DA  & $16.98$                   & $15.30$                          & \textbf{$\bf16.93$}                 & $15.91$                     \\
All & $19.54$                   & $17.99$                         & \textbf{$\bf19.60$}                  & $18.50$                      \\\hline
    & \multicolumn{4}{c}{$20$ $\leq$ Sequence  length $\leq$ $10$}                                                                                                                                                                  \\\hline
MSA & $26.37$                   & $24.51$                         & \textbf{$\bf27.05$}                 & $26.39$                     \\
DA  & $14.76$                   & $12.81$                         & \textbf{$\bf15.36$}                 & $14.50$                      \\
All & $18.37$                   & $16.32$                         & \textbf{$\bf18.84$}                 & $18.10$                      \\\hline
    & \multicolumn{4}{c}{$20$ $<$ Sequence  length }                                                                                                                                                                       \\\hline
MSA & $18.27$                   & $15.09$                         & \textbf{$\bf19.11$}                 & $17.90$                      \\
DA  & $10.65$                   & $8.54$                          & \textbf{$\bf11.21$}                 & $10.19$                     \\
All & $13.68$                   & $11.15$                         & \textbf{$\bf14.34$}                 & $13.41$                   \\\toprule 
\end{tabular}%
\caption{Sequence  length  based results on  ARGEN\textsubscript{MT}  Dev datasets. }
\label{tab:seq_length_dev}
}
\end{table}


